Fullerenes, Zero-modes, and Self-adjoint Extensions

We consider the low-energy electronic properties of graphene cones in the presence of a global Fries-Kekul\'e Peierls distortion. Such cones occur in fullerenes as the geometric response to the disclination associated with pentagon rings. It is well known that the long-range effect of the disclination deficit-angle can be modelled in the continuum Dirac-equation approximation by a spin connection and a non-abelian gauge field. We show here that to understand the bound states localized in the vicinity of a pair of pentagons one must, in addition to the long-range topological effects of the curvature and gauge flux, consider the effect the short-range lattice disruption near the defect. In particular, the radial Dirac equation for the lowest angular-momentum channel sees the defect as a singular endpoint at the origin, and the resulting operator possesses deficiency indices $(2,2)$. The radial equation therefore admits a four-parameter set of self-adjoint boundary conditions. The values of the four parameters depend on how the pentagons are distributed and determine whether or not there are zero modes or other bound states.

==> mma_defs.tex <==
\def\hbn{{\hfil\break\noindent}}
\def\opt{{\bf (optional)\/}}
\def\bi{\begin{itemize}}
\def\ei{\end{itemize}}
\def\bea{\begin{eqnarray}} 
\def\eea{\end{eqnarray}}
\def\be{\begin{equation}}
\def\ee{\end{equation}}
%\def\be{\[}	%...begin un-numbered equation 
%\def\ee{\]}     %...end   un-numbered equation
\def\line{\hbox to \hsize}    
\def\frac #1#2{{#1\over #2}}
\def\Tr{{\rm  Tr\,}}
\def\tr{{\rm  tr\,}}
\def\Psid{\Psi^{\dagger}} 
\def\psid{\psi^{\dagger}}
\def\bpsi{{\overline \psi}}
\def\bzeta{{\overline\zeta}}
\def\bareta{{\overline\eta}}
\def\bxi{{\overline\xi}}
\def \bz{{\overline z}} 
\def\phid{\varphi^*}
\def\ad{ a^{\dagger}} 
\def\bd{ b^{\dagger}}    
\def\Z{{\cal Z}}
\def\hH{{\hat H}}
\def\sgn{{\rm sgn\,}}
\def\det{{\rm det\,}}
\def\Det{{\rm Det\,}}
\def\dim{{\rm dim\,}}
\def\A{{\bf A}}
\def\B{{\bf B}} 
\def\T{{\bf T}}
\def\I{{\bf I}}
\def\P{{\bf P}}
\def\a{{\bf a}}
\def\b{{\bf b}}
\def\c{{\bf c}}
\def\d{{\bf d}}
\def\e{{\bf e}}
\def\f{{\bf f}}
\def\g{{\bf g}}
\def\r{{\bf r}}
\def\n{{\bf n}}
\def\x{{\bf x}}
\def\y{{\bf y}}
\def\z{{\bf z}}
\def\V{{\bf v}}
\def\w{{\bf w}}
\def\barph{{\overline\varphi}}
\def\ket #1{{\vert #1\rangle}}
\def\bra #1{{\langle #1\vert}}
\def\brak #1#2{{\langle#1, #2\rangle}}
\def\eval #1#2#3{{\langle#1\vert#2\vert#3\rangle}} 
\def\vev #1{{\langle #1\rangle}}
\def\1{\mbox{\bf I}}
\def\Re{{\rm Re}\,}
\def\Im{{\rm Im}\,}
\def\grad{{\rm grad\,}}
\def\curl{{\rm curl\,}}
\def\div {{\rm div\,}}
\def\pr{^\prime}
\def\vec#1{{\bf#1}}
\def\eg{{\sl e.g.\/}}
\def\ie{{\sl i.e.\/}}
\def\viz{{\sl viz.\/}}
\def\etc{{\sl etc.\/}}
\def\sech{{\rm sech\,}}
\def\tanh{{\rm tanh\,}}
\def\DPS{\displaystyle}
\def\cosec{{\rm cosec\,}}
%-----------------------------------------------------------
\def\cfo{\bf}
\def\mhe{{\cfo Henkel\/}}
\def\hww{{\cfo Wyld\/}}
\def\lva{{\cfo Ahlfors\/}}
\def\trn{{\cfo Needham\/}}
\def\hap{{\cfo Priestley\/}}
\def\mja{{\cfo Ablowitz \&\ Fokas\/}}
\def\ckp{{\cfo Carrier et al.\/}}
\def\cmb{{\cfo Bender \&\ Orszag\/}}
\def\dak{{\cfo Dennery \&\ Krzywicki\/}}
\def\hfj{{\cfo Jones\/}}
\def\rhb{{\cfo Riley et al.\/}}
\def\maw{{\cfo Mathews \&\ Walker\/}}
\def\hog{{\cfo Georgi\/}}
\def\bm#1{\mbox{\boldmath$#1$}} 
%----------------------------------------------------
%Environments
%--------------------------------------------------

\newenvironment{Quote}% Definition of new quote
{\begin{list}{}{%
\setlength{\leftmargin}{10 pt}
\setlength{\rightmargin}{\leftmargin}}
\item[]}
{\end{list}}

\newenvironment{Exercise} % definition of Exercise environment
     {\refstepcounter{exercisenumber} \begin{Quote}\small{\sl
     Exercise~\thechapter.\theexercisenumber\/}:}
{\end{Quote}}

\newenvironment{Example} % definition of Example environment     
{\begin{Quote}\small{\sl Example\/}:}
{\end{Quote}}

%-----------------------------------------------------------
%-----------------
%       ...see LaTeX/p.185
%       ...end with \end{list}
\def\levelonelist{
        \begin{list}{\mybulA}%
                        {
        \setlength{\topsep}{0pt}
        \setlength{\parsep}{0pt}
        \setlength{\partopsep}{0pt}
        \setlength{\itemsep}{0pt}
                        }
                }
%-----------------
%       ...see LaTeX/p.185
%       ...end with \end{list}
\def\leveltwolist{
        \begin{list}{\mybulB}%
                        {
        \setlength{\topsep}{0pt}
        \setlength{\parsep}{0pt}
        \setlength{\partopsep}{0pt}
        \setlength{\itemsep}{0pt}
                        }
                }
%-----------------
\def\bo{\levelonelist}
\def\bt{\leveltwolist}
\def\el{\end{list}}
%-----------------------------------------------------------

